Design and analysis of digital communication within an SoC-based control system for trapped-ion quantum computing

Electronic control systems used for quantum computing have become increasingly complex as multiple qubit technologies employ larger numbers of qubits with higher fidelity targets. Whereas the control systems for different technologies share some similarities, parameters like pulse duration, throughput, real-time feedback, and latency requirements vary widely depending on the qubit type. In this paper, we evaluate the performance of modern System-on-Chip (SoC) architectures in meeting the control demands associated with performing quantum gates on trapped-ion qubits, particularly focusing on communication within the SoC. A principal focus of this paper is the data transfer latency and throughput of several high-speed on-chip mechanisms on Xilinx multi-processor SoCs, including those that utilize direct memory access (DMA). They are measured and evaluated to determine an upper bound on the time required to reconfigure a gate parameter. Worst-case and average-case bandwidth requirements for a custom gate sequencer core are compared with the experimental results. The lowest-variability, highest-throughput data-transfer mechanism is DMA between the real-time processing unit (RPU) and the PL, where bandwidths up to 19.2 GB/s are possible. For context, this enables reconfiguration of qubit gates in less than 2$\mu$s, comparable to the fastest gate time. Though this paper focuses on trapped-ion control systems, the gate abstraction scheme and measured communication rates are applicable to a broad range of quantum computing technologies.

==> chapters/bio.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/bio/irtij.jpg}}]{Nafis Irtija} is a Ph.D. student and research assistant in the Department of Electrical and Computer Engineering, University of New Mexico. He received his master's in Computer Engineering from University of New Mexico, and his master's and bachelor's in Electrical and Electronic Engineering from the University of Dhaka, Bangladesh. His main research interests include Register Transfer Level design, Field Programmable Gate Arrays, System on a Chip based designs, distributed decision making based on reinforcement learning and game theory.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/bio/plusq.jpg}}]{Jim Plusquellic}
is a Professor in Electrical and Computer Engineering at the University of New Mexico. He received both his M.S. and Ph.D. degrees in Computer Science from the University of Pittsburgh. Professor Plusquellic received an "Outstanding Contribution Award" from IEEE Computer Society in 2012 and 2017 for co-founding and for his contributions to the Symposium on Hardware-Oriented Security and Trust (HOST).
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/bio/tsiro.jpg}}]{Eirini Eleni Tsiropoulou} is currently an Assistant Professor at the Department of Electrical and Computer Engineering, University of New Mexico. Her main research interests lie in the area of cyber-physical social systems and wireless heterogeneous networks, with emphasis on network modeling and optimization, resource orchestration in interdependent systems, reinforcement learning, game theory, network economics, and Internet of Things. Four of her papers received the Best Paper Award at IEEE WCNC in 2012, ADHOCNETS in 2015, IEEE/IFIP WMNC 2019, and INFOCOM 2019 by the IEEE ComSoc Technical Committee on Communications Systems Integration and Modeling. She was selected by the IEEE Communication Society - N2Women - as one of the top ten Rising Stars of 2017 in the communications and networking field. She received the NSF CRII Award in 2019 and the Early Career Award by the IEEE Communications Society Internet Technical Committee in 2019.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/bio/goldb.jpg}}]{Joshua Goldberg} is a Principal Electrical Engineer in the Photonic Microsystems Technologies Department at Sandia National Laboratories, Albuquerque, NM, USA. He received a B.S. in Electrical Engineering from Texas Tech University and an M.B.A. from the University of Phoenix. 
Joshua Goldberg has been specializing in software development over the last 22 years. His recent efforts include modernizing control software paradigms for trapped ion quantum systems to further full stack development for quantum information platforms.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/bio/lobse.jpg}}]{Daniel Lobser} leads the control systems thrust of QSCOUT. His main research interest is the development of custom classical and quantum control hardware that employs novel paradigms for coherent operations and dynamic noise mitigation in trapped-ion qubit platforms. He received his Ph.D. in physics from the University of Colorado, Boulder in 2015, where he studied ultracold atomic gases.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/bio/stick.jpg}}]{Daniel Stick} is a Distinguished Member of Technical Staff at Sandia National Labs. His research focuses on developing innovative technologies around atomic and quantum systems, including micro-fabricated surface ion traps for quantum information applications.  This work includes the design and fabrication of the traps, as well as experiments with storing, transporting, and performing quantum gates on ions.  Dr. Stick received his BS from Caltech and his PhD from the University of Michigan.  He was the recipient of a 2012 Presidential Early Career Award for Scientists and Engineers (PECASE) for his research in trapped ion quantum computing.
\end{IEEEbiography}
